Self-Consistent Recursive Diffusion Bridge for Medical Image Translation

Denoising diffusion models (DDM) have gained recent traction in medical image translation given improved training stability over adversarial models. DDMs learn a multi-step denoising transformation to progressively map random Gaussian-noise images onto target-modality images, while receiving stationary guidance from source-modality images. As this denoising transformation diverges significantly from the task-relevant source-to-target transformation, DDMs can suffer from weak source-modality guidance. Here, we propose a novel self-consistent recursive diffusion bridge (SelfRDB) for improved performance in medical image translation. Unlike DDMs, SelfRDB employs a novel forward process with start- and end-points defined based on target and source images, respectively. Intermediate image samples across the process are expressed via a normal distribution with mean taken as a convex combination of start-end points, and variance from additive noise. Unlike regular diffusion bridges that prescribe zero variance at start-end points and high variance at mid-point of the process, we propose a novel noise scheduling with monotonically increasing variance towards the end-point in order to boost generalization performance and facilitate information transfer between the two modalities. To further enhance sampling accuracy in each reverse step, we propose a novel sampling procedure where the network recursively generates a transient-estimate of the target image until convergence onto a self-consistent solution. Comprehensive analyses in multi-contrast MRI and MRI-CT translation indicate that SelfRDB offers superior performance against competing methods.

==> contents/theory_arc.tex <==
\section{Theory}zoo
% where $p_{\text{target}}$ and $p_{\text{prior}}$ are marginals at $t=0$ and $t=T$ respectively \cite{chen2023likelihood}.

\subsection{Diffusion Bridges}
Diffusion Bridges (DB) – as an entropy-regularized optimal transport problem – seeks two optimal policies that transform back-and-forth between two arbitrary distributions, i.e. $p_{data}$ and $p_{prior}$, in a finite horizon \cite{sch1932theorie}. The transformation can be achieved through the forward and backward SDE respectively:
%
\begin{subequations} \label{eq:SB-SDE}
\begin{align}
dX_t &= [f + g^2 \nabla \log \Psi(t, X_t)]dt + g dW_t, \: X_0\sim p_{\text{data}} \label{eq:SDE_forward}\\
dX_t &= [f - g^2 \nabla \log \hat{\Psi}(t, X_t)]dt + g \bar{dW_t}, \: X_T\sim p_{\text{prior}} \label{eq:SDE_backward}
\end{align}
\end{subequations}
%
where $\nabla \log \Psi(t, X_t)$ and $\nabla \log \hat{\Psi}(t, X_t)$ are the optimal forward and backward drifts for DB. Also, $ X_0 \sim p_{\text{target}}$ and $X_T \sim p_{\text{prior}}$ are boundary distributions \cite{chen2023likelihood},\cite{debortoli2023diffusion}. 
The optimality can be characterized with two PDEs that are coupled through boundary conditions:
% 
\begin{subequations} \label{eq:SB-PDE}
\begin{align}
\frac{\partial \Psi(x,t)}{\partial t} &= -\nabla \Psi^{\top} f - \frac{1}{2}\beta \Delta \Psi, \\
\frac{\partial \hat{\Psi}(x,t)}{\partial t} &= -\nabla \cdot (\hat{\Psi} f) + \frac{1}{2}\beta \Delta \hat{\Psi}, \\
\Psi(x, 0) \hat{\Psi}(x, 0) &= p_{data}(x), \quad \Psi(x, 1) \hat{\Psi}(x, 1) &= p_{prior}(x)
\end{align}
\end{subequations}

DDMs are a special cases of diffusion bridges. In DDM, $p_{prior}$ is assumed to be an isotropic Gaussian distribution, $ \mathcal{N}(0, I)$ \cite{DDPM}. Subsequently, DDM defines the following forward SDE:
\begin{equation} \label{eq:DDM_forward}
    dX_t = fdt + g dW_t, \: X_0\sim p_{\text{data}}
\end{equation}
It is simplified further with $f(x, t) = -\frac{1}{2}\beta(t)x$ and $g(t) = \sqrt{\beta(t)}$ \cite{song2020score}. Nelson's duality for DDMs marginal distribution can be expressed as $p(x,t) = \Psi(x,t)\hat{\Psi(x,t)}$ \cite{nelson2020}. Thus, $\nabla \log \Psi(t, X_t) - \nabla \log p(t, X_t) = \nabla \log \hat\Psi(t, X_t)$, if we substitute this in \ref{eq:SDE_backward}:
\begin{equation}
            dX_t = [f + g^2 \nabla \log\Psi(t, X_t) - g^2 \nabla \log p]dt + g \bar{dW_t} \label{eq:Score_reverse}
\end{equation}
To equate Equation \ref{eq:SDE_forward} and \ref{eq:DDM_forward}, $\nabla \log \Psi(t, X_t)$ have to be $0$. Then reverse equation \ref{eq:Score_reverse} becomes, $dX_t = [f - g^2 \nabla \log p]dt + g \bar{dW_t}$ which is exactly the reverse time SDE for \ref{eq:DDM_forward} that is defined by \cite{Anderson1982}. 

%It is resulted as following forward process:
%\begin{equation}
%    x_i = \sqrt{1-\beta_i}x_{i-1} + \sqrt{\beta_i}z_{i-1}
%\end{equation}
%where $z_i \sim \mathcal{N}(0,1)$. Thus, forward process is a Markov chain perturbation Gaussian kernel $p(\mathbf{x}_t|\mathbf{x}_{t-1}) := \mathcal{N}(\mathbf{x}_t; \sqrt{1-\beta_t}\mathbf{x}_{t-1}, \beta_t \mathbf{I})$. For any given time $t$:
%\begin{equation}
%    p_{i} (\mathbf{x}_i | \mathbf{x}_0) = \mathcal{N}(\mathbf{x}_i; \sqrt{\alpha_i}\mathbf{x}_0, (1 - \alpha_i)\mathbf{I})
%\end{equation}
%where $\alpha_i := \prod_{j=1}^{i} (1 - \beta_j)$. 
%Then its reverse process time can be solved by:
%\begin{equation}
%    p_{data} = p_{prior} \prod_{t=1}^{T} p_\theta (\mathbf{x}_{t-1}|\mathbf{x}_t)
%\end{equation}
%where $\p_\theta$ is unknown reverse time transition kernel. Reverse process is also connected to 
% explain nonlinear diffusion
%The forward process, as described by Equation \ref{eq:SB-SDE}, incorporates the term $\nabla \log \Psi(t, X_t)$. This term introduces a nonlinear forward drift, absent in linear diffusion scenarios such as those found in Score-Based Generative Models (SGM) \cite{song2020score}. The nonlinearity of this term enables the process to transport samples beyond the Gaussian Prior.
%Maybe draw an overall conculsion of SB??
\subsection{SelfRDB}

\begin{figure*}[t]
\begin{minipage}{0.7\textwidth}
{\includegraphics[width=0.97\columnwidth]{figures/method.pdf}}
\end{minipage}
\begin{minipage}{0.3\textwidth}
\caption{
    Explanation of method.
}
\label{fig:method}
\end{minipage}
\hfill
\end{figure*}

\textbf{terter}We propose a novel SB method for high-fidelity and robust translation between source and target modalities of a given anatomy. 
% SelfRDB employs SB with an improved scheduling model. Architectural imporvments.
\subsubsection{Diffusion Bridge Design}
Finding direct solution to \ref{eq:SB-SDE} is intractable due to the coupling of $\Psi(x, .)$ and $ \hat{\Psi}(x, .)$. By inspiring from \cite{liu2023i2sb}, we implement a tractable novel transportation model. 


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/forward2.pdf}
    \caption{UNK}
    \label{fig:scheduler}
\end{figure}

SC-RDB forward process $q(t,x)$ can be defined as follows:
\begin{subequations} \label{eq:raw_sch}
    \begin{gather}
    \mu_{x_0,t} = \frac{\bar{\sigma}_t^2}{\bar{\sigma}_t^2 + \sigma_t^2} \label{eq:raw_sch_a} \\
    \mu_{y,t} = \frac{\sigma_t^2}{\bar{\sigma}_t^2 + \sigma_t^2} \label{eq:raw_sch_b} \\
    \delta_t^2 = \frac{\sigma_t^2}{\bar{\sigma}_t^2 + \sigma_t^2} \label{eq:raw_sch_c} \\
    q(X_t| X_0, X_T) \coloneq \mathcal{N}(X_t; \mu_{x_0,t} X_0 + \mu_{y,t} X_T, \delta_t^2 I) \label{eq:raw_sch_d}
    \end{gather}
\end{subequations}


where $\quad \sigma_t^2 \coloneqq \int_0^t g(\tau) d\tau \quad$ and $\quad \bar{\sigma}_t^2 \coloneqq \int_t^T g(\tau) d\tau$ are analytic marginal variances of the \ref{eq:SB-SDE} when \(f \coloneq 0\) \cite{liu2023i2sb}. \(f \coloneq 0\) is reasonable when we consider that f is affine  for Gaussian transition kernels \cite{song2020score} then it can be encapsulated into nonlinear part of the equations in \ref{eq:SB-SDE} and let network learn it if it different than 0.

In SC-RDB framework we defined the diffusion function $g(t)$ as follows:
\begin{equation}
g(t;\phi) = \left(\left(\frac{T}{2}-\left|{t-\frac{T}{2}} \right|\right)\frac{\sqrt{\frac{\phi}{T}}}{T-1}\right)^2
\end{equation}
where $\phi$ is an hyperparameter that controls the noise level at each time step. The diffusion coefficients are symmetric with respect to $T/2$ and always positive.  


Even though current assumptions and constructed framework boil downs to \ref{eq:raw_sch} it has one important deficit. At any given time $X_t$ is a Gaussian distribution with a given mean and distribution at \ref{eq:raw_sch}. It is observed that variance scheduler maximized at the $t=T/2$ (see Appendix \ref{app:var_max_point}). Therefore, it starts from pure source then gradually make it noisy blending with target image up until $t=T/2$. For $X_{T/2}$ most of the information lost to the Gaussian noise. Therefore, empirically it is observed that real iterative correction (reverse diffusion) takes place after T/2. Even if the model went very bad up-until at $t=T/2$, it restarts at $t=T/2$.
% By using this insight variance scheduler $\delta_t^2$ modified as follows:
% \begin{equation} \label{eq:new_var}
%     \delta_t^2 = \frac{\sigma_t^2}{\bar{\sigma}_t^2 + \sigma_t^2}
% \end{equation}
with this definition variance function shape become exponential instead of a bell shape curve. By this new definition, resolved the issue about inefficiency in the first half of the reversing process. Overall mean and variance schedulers \ref{eq:raw_sch_a},\ref{eq:raw_sch_b}, \ref{eq:raw_sch_c} used in \ref{eq:raw_sch_d} support the ancestral sampling \cite{liu2023i2sb}. Thus, it can be define analytically (see Appendix \ref{app:PosteriorSampling}).


SC-RDB is indeed more than a abstract mathematical framework. We are diffusing a source image in addition to Gaussian kernel such that at each step data has a part of target image and source image in it. Three coefficient required by the SC-RDB can be seen from the bottom of the Figure \ref{fig:scheduler}. $X_t$ is consists of $\mu_{x_0,t} X_0 + \mu_{y,t} y + \delta_t \mathcal{N}(0,1)$ as seen from to top of the Figure \ref{fig:scheduler}. SGM like frameworks requires certain conditions like sufficiently small steps with high number of steps to end up the prior (pure Gaussian Noise) \cite{song2020score}. SC-RDB guarantees the convergences to the desired prior for a given T without a conditioning on step size or number of steps.  

% There is inconsistency between X_T and y usage. They are indeed same thing. 
% I'll change the alpha notation. 
\subsubsection{Adversarial Diffusion Process}
In SC-RDB, For a generation with equation \ref{eq:posterior}, at each step a $\Tilde{X_0}$ is required such that $\Tilde{X_0} \approx X_0$. Indeed this process again a denoising process just like SGM such that with reverse time diffusion $p_{prior}$ mapped to $p_{target}$. However, SC-RDB frame work requires more complex denoising steps. Therefore, to capture complex transition in each step, as a part of SelfRDB architecture we introduce a novel source-conditional adversarial projector, as inspired by a recent report on unconditional generation of natural images using adversarial learning \cite{DiffNvidia}. 

SelfRDB generator $G_\theta(X^*_t,y,t,z)$ predicts $\Tilde{X_0}$ for each time steps (see \ref{sec:network} for details about generator architecture) and trained as adversarial. This method has to important merits. Firstly, as reported \cite{DiffNvidia}, it can capture more complex transition between steps. Secondly, Equation \ref{eq:posterior} requires a close prediction of $X_0$ reverse diffusion, thus directly $X_0$ prediction well suited for SC-RDB framework. Furthermore, it is mostly harmonic with our novel architecture improvement self-conditioning which will be explained at Section \ref{sec:selfcond}.

To train $G_\theta$ with adversarial loss, a discriminator $D_\theta((\Tilde{X_t} \text{or} X_t), X_{t+1}, t)$ distinguishes samples drawn from estimated versus true distributions. A non-saturating adversarial loss with gradient penalty is adopted for $G_\theta$ \cite{mescheder2018training}:
\begin{align} \label{eq:D-loss} 
&&L_{D_{\boldsymbol{\theta}}} = \mathbb{E}_{t,q(\boldsymbol{X}_t|\boldsymbol{X}_0, \boldsymbol{y})}  \left[ -log(D_{\boldsymbol{\theta}}(\boldsymbol{X}_{t})) \right]  \notag \\
&&+ \mathbb{E}_{q(\boldsymbol{X}_{t}|\boldsymbol{X}_{t-1}, \boldsymbol{\Tilde{X_0}})} [ -log(1-D_{\boldsymbol{\theta}}(\Tilde{}{\boldsymbol{X}}_{t})) ]  \notag \\ 
&&\left. + \eta \mathbb{E}_{q(\boldsymbol{X}_{t}|\boldsymbol{X}_{0},\boldsymbol{y})} \left\| \nabla_{\boldsymbol{X}_{t}} D_{\boldsymbol{\theta}}(\boldsymbol{X}_{t})  \right\|^2_2  \right]  
\end{align}
where $\eta$ is the weight for the gradient penalty.

Additionally, L1 reconstruction loss is introduced which makes final training loss as follows:
\begin{equation}
    L = L_{D_{\boldsymbol{\theta}}} + \lambda \left | X_0 - \Tilde{X_0} \right |
\end{equation}
where $\lambda$ is the weight coefficient for L1 loss. 


% Discriminator q(t-1|t)den haberdar ediyor. 
\subsubsection{Self-conditioning} \label{sec:selfcond}
% explain how self-condition improves x0 preds.
% Source conditioning at each step

\subsubsection{Learning Procedures}
% beta choice


==> contents/theory_v1.tex <==
\section{Theory and Methods}
% where $p_{\text{target}}$ and $p_{\text{source}}$ are marginals at $t=0$ and $t=T$ respectively \cite{chen2023likelihood}.

\subsection{Diffusion Bridges}
Diffusion bridges are a general framework to describe the evolution between two arbitrary probability distributions across a finite time interval $t \in [0,T]$ \cite{liu2023i2sb}. In the context of source-to-target mapping, the learning objective for diffusion bridges can be expressed as:
%
\begin{equation}
\min _{p \in \mathcal{P}_{[0,T]}} D_\text{KL}(p \| q), \quad \text{s.t.} \; p_0=p_{\text {target}}, p_T=p_{\text {source}}
\label{eq:sb_kl}
\end{equation}
%
where $\mathcal{P}_{[0,T]}$ is the space of path measures with marginal densities $p_0=p_{\text {target }}$ and $p_T=p_{\text {source}}$ as boundary conditions and $q$ is the \textit{reference path measure}. %The optimality condition to the SB objective is defined by two PDEs (see Appendix ?). Subsequently, the solution to \eqref{eq:sb_kl} is given by the \textit{optimal path measure} $p^* \in \mathcal{P}_{[0,T]}$ which is induced by the following forward-backward SDEs \cite{chen2021likelihood}:
%
\begin{subequations} \label{eq:SB-SDE}
\begin{align}
\mathrm{d}\boldsymbol{x}_t &= [\boldsymbol{f} + g^2 \nabla \log \Psi(\boldsymbol{x}_t, t)]\mathrm{d}t + g \mathrm{d}\boldsymbol{w}_t, \: \boldsymbol{x}_0\sim p_{\text{target}} \label{eq:SDE_forward}\\
\mathrm{d}\boldsymbol{x}_t &= [\boldsymbol{f} - g^2 \nabla \log \hat{\Psi}(\boldsymbol{x}_t, t)]\mathrm{d}t + g {\mathrm{d}\bar{\boldsymbol{w}}_t}, \: \boldsymbol{x}_T\sim p_{\text{source}} \label{eq:SDE_backward}
\end{align}
\end{subequations}
%
where $\nabla \log \Psi(\boldsymbol{x}_t, t)$ and $\nabla \log \hat{\Psi}(\boldsymbol{x}_t, t)$ are nonlinear forward and backward drifts, as opposed to diffusion models with linear drift \cite{song2020score, DDPM}. Consequently, SB generalizes beyond Gaussian priors. Yet, the solution to SB is intractable and requires iterative methods (e.g. IPF \cite{kullback1968probability}) having scalability issues due to significant computational cost.

A tractable class of SB \cite{liu2023i2sb} leverages the Nelson's duality \cite{nelson1967} to relate the nonlinear drift terms $\nabla \log \Psi(\boldsymbol{x}_t, t)$ and $\nabla \log \hat{\Psi}(\boldsymbol{x}_t, t)$ to the score function $\nabla \log p(\boldsymbol{x}_t, t)$ which indicates that SB generalizes diffusion models theoretically. Yet, the tractability is ensured by the assumption that the boundary distribution $p_0$ is a Dirac delta distribution, i.e. $p_0(\cdot) := \delta_x (\cdot)$. This implies that for a given data pair, $(\boldsymbol{x}_0, \boldsymbol{x}_T)$, the marginal density is evaluated such that $p_0(\boldsymbol{x}_0) = 1$. This assumption decouples constraints within the PDEs (see Appendix ?), ensuring that the boundary distributions become computationally tractable.

Diffusion bridges established upon SB formulation have unrestricted prior distribution and hence an ideal alternative for diffusion models specifically in cases where prior knowledge significantly influences the model's behavior.
%





\begin{figure*}[t]
\begin{minipage}{0.7\textwidth}
{\includegraphics[width=0.97\columnwidth]{figures/method.pdf}}
\end{minipage}
\begin{minipage}{0.3\textwidth}
\caption{SelfRDB casts a diffusion bridge to transform between source and target images of an anatomy. \textbf{A)} In the forward process, the start-point $x_0$ is taken as the target image and the end-point $x_T$ is taken as a noise-added version of the source image $y_{\epsilon}=y+\epsilon$. Intermediate image samples are derived via the forward transition probability $q(x_t | x_{t-1},y)$, whose mean is a convex combination of target-source images, and whose noise-driven variance increases towards $t=T$. In the reverse process, sampling is initiated on $x_T=y_{\epsilon}$, and intermediate samples are derived via the reverse transition probability $p_{\theta}(x_{t-1} | x_{t},y_{\epsilon})$. \textbf{B)} Reverse diffusion steps are operationalized via a recovery network $G_{\theta}(x_t,t,y,\tilde{x}_0^r)$ that recursively generates a target-image estimate $\tilde{x}_0^{r+1}$ at the current timestep, given the target-image estimate from the previous recursion $\tilde{x}_0^{r}$ and the original source image $y$. Recursions are stopped upon convergence onto a self-consistent solution $\tilde{x}_0=G_{\theta}(x_t,t,y,\tilde{x}_0)$, which is then used for posterior sampling of $\hat{x}_{t-1}$ according to the normal distribution $q(x_{t-1}|x_t,\tilde{x}_0)$. To improve posterior sampling, a discriminator subnetwork $D_{\theta}(x_{t-1} \mbox{ or } \hat{x}_{t-1},t,x_t)$ is used to perform adversarial learning on the recovered sample $\hat{x}_{t-1}$.}
\label{fig:method}
\end{minipage}
\hfill
\end{figure*}

\subsection{SelfRDB}

\subsubsection{Diffusion Bridge}
Existing diffusion bridges assume clean target and source image pair $(\boldsymbol{x}_0, \boldsymbol{x}_T)$ at the start and end points of the forward process such that $\boldsymbol{x}_0 \sim p_\text{target}$ and $\boldsymbol{x}_T \sim p_\text{source}$ where $p_\text{target}$ and $p_\text{source}$ are target and source distributions, respectively. In this configuration, the variance is zero at both the initial and final points of the process and it progressively increases as the process moves toward the midpoint, $t=T/2$. This setting is based on the premise that the start and end points are well-defined and deterministic, while allowing for uncertainty in the intermediate steps. The Dirac delta assumption in \cite{liu2023i2sb} restricts one side of the bridge and relaxes other side to be an arbitrary distribution. However, in the paired training configuration, the boundaries can be seen as mixtures of dual Dirac distribution \cite{chen2023schrodinger}. In this case, while the transport model with the regular diffusion bridge is optimal for the training data pairs, such variance scheduling may hinder its generalization ability for unseen source images during inference. To this end, we propose a novel diffusion bridge scheme with \textit{soft prior}. Figure \ref{fig:forward_samples} compares our forward process with that of regular diffusion process \cite{DDPM, song2020score} and existing diffusion bridges \cite{liu2023i2sb} by demonstrating sample MR images and corresponding mean-variance scheduling.

Given an image pair $(\boldsymbol{x}_0, \boldsymbol{y})$ such that $\boldsymbol{x}_0 \sim p_\text{target}$ and $\boldsymbol{y} \sim p_\text{source}$, our forward process is described by the following transition probability:
%
\begin{equation}
    q(\boldsymbol{x}_t| \boldsymbol{x}_0, \boldsymbol{x}_T) = \mathcal{N}(\boldsymbol{x}_t; \mu_{x_0,t} \boldsymbol{x}_0 + \mu_{y,t} \boldsymbol{y}, \delta_t^2 \boldsymbol{I}) \label{eq:q_sample}
\end{equation}
%
which is the analytical posterior where mean and variance schedules are defined as follows:
%
\begin{subequations} \label{eq:schedule}
    \begin{gather}
    \mu_{x_0,t} = \frac{\bar{\sigma}_t^2}{\bar{\sigma}_t^2 + \sigma_t^2}, \quad 
    \mu_{y,t} = \frac{\sigma_t^2}{\bar{\sigma}_t^2 + \sigma_t^2} \label{eq:mean_schedule} \\
    \delta_t^2 = \frac{\sigma_t^2}{\bar{\sigma}_t^2 + \sigma_t^2} \label{eq:var_schedule}
    \end{gather}
\end{subequations}
%
where $\sigma_t^2 \coloneqq \int_0^t g(\tau) d\tau$ and $\bar{\sigma}_t^2 \coloneqq \int_t^T g(\tau) d\tau$ are accumulated variances. Subsequently, we define the following diffusion coefficient:
%
\begin{equation}
g_t(\phi) = \frac{(T-|2 t-T|)^2 \phi}{4 T(T-1)^2}
\label{eq:diff_coeff}
\end{equation}
%
where $\phi$ is an hyperparameter that controls the noise level at each timestep. The diffusion coefficient is symmetric with respect to $t = T/2$ and always positive, i.e. $g_t(\phi) > 0$.  

% connect to SGM's perturbations for low density vector field regions

In contrast to regular diffusion bridges, our novel scheduling scheme establishes the bridge between clean target images and noisy source images. As demonstrated in Figure \ref{fig:soft_prior}, regular diffusion bridge maps a target to its exact source pair following a stochastic path. On the other hand, our diffusion bridge maps a target to a point in the vicinity of its source pair. Specifically, our transport model concerns with the evolution between the data pair $(\boldsymbol{x}_0, \boldsymbol{x}_T)$ such that $\boldsymbol{x}_0 \sim p_\text{target}$ and $\boldsymbol{x}_T \sim \mathcal{N}(\boldsymbol{y}, \epsilon^2 \boldsymbol{I})$ where $\boldsymbol{y} \sim p_\text{source}$ is a clean target image and $\boldsymbol{x}_T$ is its noisy version. Consequently, we define the \textit{soft prior} $p_\text{source} \coloneq \mathcal{N}(\boldsymbol{y}, \epsilon^2 \boldsymbol{I})$. 

In reverse direction as shown in Figure \ref{fig:soft_prior}, a given source sample may correspond to a low-density region of the score function, $\nabla \log \Psi(\boldsymbol{x}_t, t)$, of the reverse SDE. In this scenario, translation from source to target yields inaccurate results. To overcome this limitation, SelfRDB leverages the noise perturbation technique \cite{song2019generative} to improve the diffusion bridge: our soft prior smooths the source distribution through Gaussian perturbations, effectively reducing the likelihood that any given source sample falls into a low-density area. Therefore, this novel bridge configuration improves generalization ability of the model beyond training image pairs.


\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/soft_prior.pdf}
    \caption{Diffusion models learn the score function of the data through a multi-step transformation between the start- and end-points of the underlying process. Image samples are typically corrupted with Gaussian noise that smooths the data distribution by discarding some of the original image features. Smoothing enables more uniform coverage of the data space in order to boost generalization performance. \textbf{Regular diffusion bridges} use zero noise variance at the end-point constraining them to a Dirac-delta distribution centered on the source images within the training set. This can compromise generalization performance to source images outside the training set (see red-colored dashed path). \textbf{SelfRDB} instead uses monotonically-increasing variance towards the end-point, so it is trained on noise-added source images. This improves robustness against variability in source images between training and test sets (see blue-colored dashed paths.}
    \label{fig:soft_prior}
\end{figure*}

\subsubsection{Adversarial Diffusion Process}
In SC-RDB, For a generation with equation \ref{eq:posterior}, at each step a $\Tilde{X_0}$ is required such that $\Tilde{X_0} \approx X_0$. Indeed this process again a denoising process just like SGM such that with reverse time diffusion $p_{source}$ mapped to $p_{target}$. However, SC-RDB frame work requires more complex denoising steps. Therefore, to capture complex transition in each step, as a part of SelfRDB architecture we introduce a novel source-conditional adversarial projector, as inspired by a recent report on unconditional generation of natural images using adversarial learning \cite{DiffNvidia}. 

SelfRDB generator $G_\theta(X^*_t,y,t,z)$ predicts $\Tilde{X_0}$ for each timestep and trained as adversarial. This method has to important merits. Firstly, as reported \cite{DiffNvidia}, it can capture more complex transition between steps. Secondly, Equation \ref{eq:posterior} requires a close prediction of $X_0$ reverse diffusion, thus directly $X_0$ prediction well suited for SC-RDB framework. Furthermore, it is mostly harmonic with our novel architecture improvement self-conditioning which will be explained at Section \ref{sec:selfcond}.

To train $G_\theta$ with adversarial loss, a discriminator $D_\theta((\Tilde{X_t} \text{or} X_t), X_{t+1}, t)$ distinguishes samples drawn from estimated versus true distributions. A non-saturating adversarial loss with gradient penalty is adopted for $G_\theta$ \cite{mescheder2018training}:
\begin{align} \label{eq:D-loss} 
&&L_{D_{\boldsymbol{\theta}}} = \mathbb{E}_{t,q(\boldsymbol{X}_t|\boldsymbol{X}_0, \boldsymbol{y})}  \left[ -log(D_{\boldsymbol{\theta}}(\boldsymbol{X}_{t})) \right]  \notag \\
&&+ \mathbb{E}_{q(\boldsymbol{X}_{t}|\boldsymbol{X}_{t-1}, \boldsymbol{\Tilde{X_0}})} [ -log(1-D_{\boldsymbol{\theta}}(\Tilde{}{\boldsymbol{X}}_{t})) ]  \notag \\ 
&&\left. + \eta \mathbb{E}_{q(\boldsymbol{X}_{t}|\boldsymbol{X}_{0},\boldsymbol{y})} \left\| \nabla_{\boldsymbol{X}_{t}} D_{\boldsymbol{\theta}}(\boldsymbol{X}_{t})  \right\|^2_2  \right]  
\end{align}
where $\eta$ is the weight for the gradient penalty.

Additionally, L1 reconstruction loss is introduced which makes final training loss as follows:
\begin{equation}
    L = L_{D_{\boldsymbol{\theta}}} + \lambda \left | X_0 - \Tilde{X_0} \right |
\end{equation}
where $\lambda$ is the weight coefficient for L1 loss. 


% Discriminator q(t-1|t)den haberdar ediyor. 



\subsubsection{Self-conditioning} \label{sec:selfcond}

% noisy source images corresponds to a form of augmentation increasing number of training samples to be learnt hence exceeding network capacity making unrolling idea useful for eficiently increasing network capacity.

% explain how self-condition improves x0 preds.
% Source conditioning at each step

